Fully Empirical Autotuned QR Factorization For Multicore Architectures

Tuning numerical libraries has become more difficult over time, as systems get more sophisticated. In particular, modern multicore machines make the behaviour of algorithms hard to forecast and model. In this paper, we tackle the issue of tuning a dense QR factorization on multicore architectures. We show that it is hard to rely on a model, which motivates us to design a fully empirical approach. We exhibit few strong empirical properties that enable us to efficiently prune the search space. Our method is automatic, fast and reliable. The tuning process is indeed fully performed at install time in less than one and ten minutes on five out of seven platforms. We achieve an average performance varying from 97% to 100% of the optimum performance depending on the platform. This work is a basis for autotuning the PLASMA library and enabling easy performance portability across hardware systems.

==> ATTRIBNUM <==
Rapport de recherche

Le numéro 7526 a été attribué au rapport correspondant à:

Titre
    A Fully Empirical Autotuned Dense QR Factorization For Multicore Architectures
Auteur
    agullo
Contact
    Emmanuel.Agullo@inria.fr
Projet
    HIEPACS
Fichier
    main.ps

A faire maintenant

   1. Mettre ce numéro dans le source de votre rapport
          * pour le LaTex, mettre \RRNo{7526} apres le \begin{document}
   2. Renommer le fichier source du rapport en : RR-7526.tex (ou ps ou pdf suivant les cas !)
   3. Déposer celui-ci dans HAL avec les MÊMES INFORMATIONS (titre, auteur, projet)
          * Déposer dans la catégorie "Document avec référence bibliographique" > "RAPPORT"
   4. Remplir le champ "Référence interne" avec la valeur RR-7526

